Graph Directed Coalescence Hidden Variable Fractal Interpolation Functions

Fractal interpolation function (FIF) is a special type of continuous function which interpolates certain data set and the attractor of the Iterated function system (IFS) corresponding to the data set is the graph of the FIF. Coalescence Hidden-variable Fractal Interpolation Function (CHFIF) is both self-affine and non self-affine in nature depending on the free variables and constrained free variables for a generalized IFS. In this article graph directed iterated function system for a finite number of generalized data sets is considered and it is shown that the projections of the attractors on $\mathbb{R}^{2}$ is the graph of the CHFIFs interpolating the corresponding data sets.

==> references.tex <==
@ARTICLE(barnsley-86,
   AUTHOR = "M. F. Barnsley",
   TITLE = "Fractal functions and interpolation",
   JOURNAL = "Constr. Approx.",
   YEAR = "1986",
   VOLUME = "2",
   NUMBER = "4",
   PAGES = "303-329"
)
@ARTICLE(barnsley-1989,
   AUTHOR = "M. F. Barnsley",
   TITLE = "The calculus of fractal interpolation functions",
   JOURNAL = "J.  Approx.  Theory",
   YEAR = "1989",
   VOLUME = "57",
   NUMBER = "",
   PAGES = "14-34"
)
@ARTICLE(chand-2007,
   AUTHOR = "A. K. B. Chand and  G. P. Kapoor",
   TITLE = "Smoothness analysis of coalescence hidden variable fractal interpolation functions",
   JOURNAL = "Int. J. Nonlinear Sci.",
   YEAR = "2007",
   VOLUME = "3",
   NUMBER = "1",
   PAGES = "15-26"
) 
